AgentBoard: An Analytical Evaluation Board of Multi-turn LLM Agents

Evaluating Large Language Models (LLMs) as general-purpose agents is essential for understanding their capabilities and facilitating their integration into practical applications. However, the evaluation process presents substantial challenges. A primary obstacle is the benchmarking of agent performance across diverse scenarios within a unified framework, especially in maintaining partially-observable environments and ensuring multi-round interactions. Moreover, current evaluation frameworks mostly focus on the final success rate, revealing few insights during the process and failing to provide a deep understanding of the model abilities. To address these challenges, we introduce AgentBoard, a pioneering comprehensive benchmark and accompanied open-source evaluation framework tailored to analytical evaluation of LLM agents. AgentBoard offers a fine-grained progress rate metric that captures incremental advancements as well as a comprehensive evaluation toolkit that features easy assessment of agents for multi-faceted analysis. This not only sheds light on the capabilities and limitations of LLM agents but also propels the interpretability of their performance to the forefront. Ultimately, AgentBoard serves as a step towards demystifying agent behaviors and accelerating the development of stronger LLM agents.

==> paragraphs/07_impact_statements.tex <==
This paper presents work whose goal is to advance the field of Machine Learning. Potential societal implications include we allow LLM agents to access online API in tool-operation evaluation. LLM agents could access and edit online information including Google Sheet and To-do list. However, we made sure that no personal information is leaked and no generated content is distributed online during the evaluation process.

==> prompt/game24.tex <==
\begin{tcolorbox}[breakable,title=Prompt of the Game24 ]
\textbf{\textcolor{blue}{System Prompt}}\\ 
You are an master in math. Generate your next step of action after Action. Action must not be empty. e.g. Action: put down cup.\\
\begin{tikzpicture}
\draw[dashed] (0,0) -- (\linewidth,0); % 绘制一条宽度为\linewidth的虚线
\end{tikzpicture}
\textbf{\textcolor{blue}{Instruction}}\\
You are given a set of numbers and you have to combine them using the four basic operations (+, -, *, /) to get a given goal number. You can only use each number once. Every time you use two numbers, you get a new number, which must be an integer. You would use this number along with other unused number to proceed the process. Each action must follow this format:

\verb|<a> + <b>|: add two intergers a and b, substitute a, b for available number. 
 
\verb|<a> * <b>|: multiple two intergers a and b, substitute a, b for available number. 

\verb|<a> / <b>|: divide a by b, substitute a, b for available number.
 
\verb|<a> - <b>|: minus b from a, substitute a, b for available number.

\begin{tikzpicture}
\draw[dashed] (0,0) -- (\linewidth,0); % 绘制一条宽度为\linewidth的虚线
\end{tikzpicture}
\textbf{\textcolor{blue}{Examples}}\\
Goal is to get 24. Observation: Numbers left: 1, 2, 3, 4
Action: 1 * 2 

Observation: Numbers left: 3, 4, 2

Action: 3 * 4 

Observation: Numbers left: 2, 12

Action: 2 * 12 

Observation: Numbers left: 24. Goal reached!

\end{tcolorbox}
\begin{figure}[!h]
    \vspace{0.01cm}
    \caption{Prompt for the task of Game24.}
    \label{fig:alfworld_prompt}
\end{figure}

==> prompt/movie.tex <==
\begin{tcolorbox}[breakable,title=Prompt Details for Movie]
\textbf{\textcolor{blue}{System Prompt}}\\ 
You can use actions to help people solve problems.\\
\begin{tikzpicture}
\draw[dashed] (0,0) -- (\linewidth,0); % 绘制一条宽度为\linewidth的虚线
\end{tikzpicture}
\textbf{\textcolor{blue}{Instruction}}\\
We detail name, description, input(parameters) and output(returns) of each action as follows:\\
Name: get\_search\_movie(movie\_name)\\
Description: Search for a movie by name and return basic details\\
Parameters:\\
- movie\_name (Type: string): The name of the movie to search for.\\
Returns:\\
- id : The ID of the found movie.\\
- overview : The overview description of the movie.\\
- title : The title of the movie.\\

Name: get\_movie\_details(movie\_id)\\
Description: Get detailed information about a movie by ID\\
Parameters:\\
- movie\_id (Type: string): The ID of the movie.\\
Returns:\\
- budget : The budget of the movie.\\
- genres : The genres of the movie.\\
- revenue : The revenue of the movie.\\
- vote\_average : The average vote score of the movie.\\
- release\_date : The release date of the movie.\\

Name: get\_movie\_production\_companies(movie\_id)\\
Description: Get the production companies of a movie by its ID\\
Parameters:\\
- movie\_id (Type: string): The ID of the movie.\\
Returns:\\
- production\_companies : The production companies of the movie.\\

Name: get\_movie\_production\_countries(movie\_id)
Description: Get the production countries of a movie by its ID\\
Parameters:\\
- movie\_id (Type: string): The ID of the movie.\\
Returns:\\
- production\_countries : The production countries of the movie.\\

Name: get\_movie\_cast(movie\_id)\\
Description: Retrieve the list of the top 10 cast members from a movie by its ID.\\
Parameters:\\
- movie\_id (Type: string): The ID of the movie.\\
Returns:\\
- cast : List of the top 10 cast members.\\

Name: get\_movie\_crew(movie\_id)\\
Description: Retrieve the list of crew members (limited to 10) from a movie by its ID. The list primarily includes Director, Producer, and Writer roles.\\
Parameters:\\
- movie\_id (Type: string): The ID of the movie.\\
Returns:\\
- crew : List of the top 10 of crew members\\

Name: get\_movie\_keywords(movie\_id)\\
Description: Get the keywords associated with a movie by ID\\
Parameters:\\
- movie\_id (Type: string): The ID of the movie.\\
Returns:\\
- keywords : The keywords associated with the movie.\\

Name: get\_search\_person(person\_name)\\
Description: Search for a person by name.\\
Parameters:\\
- person\_name (Type: string): The name of the person to search for.\\
Returns:\\
- id : The ID of the found person.\\
- name : The name of the person.\\

Name: get\_person\_details(person\_id)\\
Description: Get detailed information about a person by ID\\
Parameters:\\
- person\_id (Type: string): The ID of the person.\\
Returns:\\
- biography : The biography of the person.\\
- birthday : The birthday of the person.\\
- place\_of\_birth : The place of birth of the person.\\

Name: get\_person\_cast(person\_id)\\
Description: Retrieve the top 10 movie cast roles of a person by their ID\\
Parameters:\\
- person\_id (Type: string): The ID of the person.\\
Returns:\\
- cast : A list of movies where the person has acted, limited to top 10\\

Name: get\_person\_crew(person\_id)\\
Description: Retrieve the top 10 movie crew roles of a person by their ID\\
Parameters:\\
- person\_id (Type: string): The ID of the person.\\
Returns:\\
- crew : A list of movies where the person has participated as crew, limited to top 10\\

Name: get\_person\_external\_ids(person\_id)\\
Description: Get the external ids for a person by ID\\
Parameters:\\
- person\_id (Type: string): The ID of the person.\\
Returns:\\
- imdb\_id : The IMDB id of the person.\\
- facebook\_id : The Facebook id of the person.\\
- instagram\_id : The Instagram id of the person.\\
- twitter\_id : The Twitter id of the person.\\

Name: get\_movie\_alternative\_titles(movie\_id)\\
Description: Get the alternative titles for a movie by ID\\
Parameters:\\
- movie\_id (Type: string): The ID of the movie.\\
Returns:\\
- titles : The alternative titles of the movie.\\
- id : The ID of the movie.\\

Name: get\_movie\_translation(movie\_id)\\
Description: Get the description translation for a movie by ID\\
Parameters:\\
- movie\_id (Type: string): The ID of the movie.\\
Returns:\\
- translations : The description translation of the movie.\\
- id : The ID of the movie.\\

Name: check\_valid\_actions()\\
Description: Get supported actions for current tool.\\
Returns:\\
- actions (Type: array): Supported actions for current tool.\\

Name: finish(answer)\\
Description: Return an answer and finish the task\\
Parameters:\\
- answer (Type: [`string', `number', `array']): The answer to be returned\\

If you are finished, you will call ``finish" action\\
Please refer to the format of examples below to solve the requested goal. Your response must be in the format of ``Action: [your action] with Action Input: [your action input]"
\begin{tikzpicture}
\draw[dashed] (0,0) -- (\linewidth,0); % 绘制一条宽度为\linewidth的虚线
\end{tikzpicture}
\textbf{\textcolor{blue}{Examples}}\\
Goal: When did the movie Scream 6 come out?\\

Action: get\_search\_movie with Action Input: \{``movie\_name": ``Scream 6"\}\\
Observation: \{`id': 934433, `overview': `Following the latest Ghostface killings, the four survivors leave Woodsboro behind and start a fresh chapter.', `title': `Scream VI'\}\\
Action: get\_movie\_details with Action Input: \{``movie\_id": ``934433"\}\\
Observation: \{`budget': 35000000, `genres': [\{`id': 27, `name': `Horror'\}, \{`id': 53, `name': `Thriller'\}, \{`id': 9648, `name': `Mystery'\}], `revenue': 168961389, `vote\_average': 7.175, `release\_date': `2023-03-08'\}\\
Action: finish with Action Input: \{``answer": "2023-03-08"\}\\
Observation: 2023-03-08
\end{tcolorbox}
\begin{figure}[!h]
    \vspace{-0.08cm}
    \caption{Prompt Details for Movie.}
    \label{fig:movie_prompt}
\end{figure}

==> prompt/sheet.tex <==
\begin{tcolorbox}[breakable,title=Prompt Details for Sheet]
\textbf{\textcolor{blue}{System Prompt}}\\ 
You can use actions to help people solve problems.\\
\begin{tikzpicture}
\draw[dashed] (0,0) -- (\linewidth,0); % 绘制一条宽度为\linewidth的虚线
\end{tikzpicture}
\textbf{\textcolor{blue}{Instruction}}\\
We detail name, description, input(parameters) and output(returns) of each action as follows:\\
Name: open\_sheet(name)\\
Description: Open a sheet by name\\
Parameters:\\
- name (Type: string): The name of the sheet to open.\\
Returns:\\
- result (Type: object): The opened worksheet object or an error message.\\
\\
Name: del\_sheet(name)\\
Description: Deletes the specified sheet.\\
Parameters:\\
- name (Type: string): The name of the sheet to be deleted.\\
Returns:\\
- result (Type: object): Whether the operation was successful.\\
\\
Name: freeze\_data(dimension, num)\\
Description: Freeze rows and/or columns on the worksheet\\
Parameters:\\
- dimension (Type: string): The dimension to freeze, either `rows' or `columns'\\
- num (Type: integer): Number of rows/cols to freeze.\\
Returns:\\
- result (Type: object): Whether the operation was successful.\\
\\
Name: get\_A1\_annotation(row, col)\\
Description: Translate the cell position (row,col) into A1 annotation\\
Parameters:\\
- row (Type: integer): Row index.\\
- col (Type: integer): Column index.\\
Returns:\\
- result (Type: string): The A1 notation of the cell or an error message.\\
\\
Name: insert\_cols(values\_list, col\_idx)\\
Description: Insert columns into sheet at specified column index\\
Parameters:\\
- values\_list (Type: array[array[string]]): A list of lists, each list containing one column's values, which can be expressions\\
- col\_idx (Type: integer): Start column to update. Defaults to 1.\\
Returns:\\
- result (Type: object): The updated worksheet data or an error message.\\
\\
Name: insert\_rows(values\_list, row\_idx)\\
Description: Insert rows into sheet at specified row index\\
Parameters:\\
- values\_list (Type: array[array[string]]): A list of lists, each list containing one row's values, which can be expressions\\
- row\_idx (Type: integer): Start row to update. Defaults to 1.\\
Returns:\\
- result (Type: object): The updated worksheet data or an error message.\\
\\
Name: delete\_batch\_data(dimension, index\_list)\\
Description: Delete a batch of data in the sheet\\
Parameters:\\
- dimension (Type: string): The dimension to delete, either `row' or `col'.\\
- index\_list (Type: array[integer]): List of the indexes of rows/cols for deletion.\\
Returns:\\
- result (Type: object): The updated worksheet data or an error message.\\
\\
Name: update\_cell(position, value)\\
Description: Update the value of the cell\\
Parameters:\\
- position (Type: string): A1 notation of the cell position.\\
- value: The value to set.\\
Returns:\\
- result (Type: object): The updated worksheet data or an error message.\\
\\
Name: update\_cell\_by\_formula(start\_position, end\_position, position\_list, result\_position, operator)\\
Description: Update the value of the target cell by applying formulas on some specified cells. Note: Either specify position\_list or start\_position and end\_position.\\
Parameters:\\
- start\_position (Type: string): The starting position of the range. Default: `B1'.\\
- end\_position (Type: string): The ending position of the range. Default: `D2'.\\
- position\_list (Type: array[string]): A list of cell positions in A1 notation.\\
- result\_position (Type: string): The position of the cell where the result of the formula will be stored in. Default: `G2'.\\
- operator (Type: string): The operator to be applied on selected cells. Choose one from [`SUM', `AVERAGE', `COUNT', `MAX', `MIN', `MINUS', `PRODUCT'].\\
Returns:\\
- result (Type: object): The updated worksheet data or an error message.\\
\\
Name: update\_range(start\_position, end\_position, values\_list)\\
Description: Update a range of the cells from a list\\
Parameters:\\
- start\_position (Type: string): A1 notation of the start cell.\\
- end\_position (Type: string): A1 notation of the end cell.\\
- values\_list (Type: array[array[Any]]): List of values to be inserted, which can be expressions\\
Returns:\\
- result (Type: object): The updated worksheet data or an error message.\\
\\
Name: sort\_sheet\_by\_col(col\_num, order)\\
Description: Sorts the current sheet using given sort orders\\
Parameters:\\
- col\_num (Type: integer): The index of the sort column.\\
- order (Type: string): The sort order. Possible values are `asc' or `des'.\\
Returns:\\
- result (Type: object): The updated worksheet data or an error message.\\
\\
Name: merge\_cells(start\_position, end\_position)\\
Description: Merge cells in sheet\\
Parameters:\\
- start\_position (Type: string): Starting cell position(top left) in A1 annotation.\\
- end\_position (Type: string): Ending cell position(bottom right) in A1 annotation.\\
Returns:\\
- result (Type: object): The updated worksheet data or an error message.\\
\\
Name: update\_note(position, content)\\
Description: Update a note in a certain cell\\
Parameters:\\
- position (Type: string): cell position in A1 annotation.\\
- content (Type: string): The text note to insert.\\
Returns:\\
- result (Type: string): The updated note or an error message.\\
\\
Name: get\_all\_values()\\
Description: Display all cell values in current sheet\\
Returns:\\
- result (Type: array[array[Any]]): Return all cell values or an error message.\\
\\
Name: get\_range\_values(start\_position, end\_position)\\
Description: Returns a list of cell data from a specified range.\\
Parameters:\\
- start\_position (Type: string): Starting cell position in A1 annotation.\\
- end\_position (Type: string): Ending cell position in A1 annotation.\\
Returns:\\
- result (Type: array[array[Any]]): List of cell data from the specified range or an error message.\\
\\
Name: get\_cell\_value(position)\\
Description: Get the value of a specific cell\\
Parameters:\\
- position (Type: string): Cell position in A1 annotation.\\
Returns:\\
- result : Cell value or an error message.\\
\\
Name: get\_value\_by\_formula(start\_position, end\_position, position\_list, operator)\\
Description: Calculate a value applying formulas on specified cells. Note: Either specify position\_list or start\_position and end\_position.\\
Parameters:\\
- start\_position (Type: string): The starting position of the range. Default: `B1'.\\
- end\_position (Type: string): The ending position of the range. Default: `D2'.\\
- position\_list (Type: array[string]): A list of cell positions in A1 notation.\\
- operator (Type: string): The operator to be applied on selected cells. Choose one from [`SUM', `AVERAGE', `COUNT', `MAX', `MIN', `MINUS', `PRODUCT'].\\
Returns:\\
- result (Type: string): Calculated result or an error message.\\
\\
Name: filter\_cells(query, in\_row, in\_column)\\
Description: Find all cells matching the query, return all cells' position.\\
Parameters:\\
- query (Type: [`string', `re.RegexObject']): A string to match or compiled regular expression.\\
- in\_row (Type: [`integer', `None']): Row number to scope the search. Default is all rows\\
- in\_column (Type: [`integer', `None']): Column number to scope the search. Default is all columns\\
Returns:\\
- result (Type: array[string]): List of cell addresses that match the query or an error message.\\
\\
Name: get\_note(position)\\
Description: Get the note at the certain cell, or return empty string if the cell does not have a note.\\
Parameters:\\
- position (Type: string): Cell position in A1 annotation.\\
Returns:\\
- result (Type: string): Note content or an error message.\\
\\
Name: finish()\\
Description: Return an answer and finish the task\\
Returns:\\
- result (Type: array[array[Any]]): Return all cell values or an error message.\\


\begin{tikzpicture}
\draw[dashed] (0,0) -- (\linewidth,0); % 绘制一条宽度为\linewidth的虚线
\end{tikzpicture}
\textbf{\textcolor{blue}{Examples}}\\
Goal: ``Sheet90'' saves the clothing inventory information, please delete items with price changed by more than 25\%, update the price of other items.\\
\\
Action: get\_all\_values with Action Input: \{\}\\
Observation: [[`Category', `Brand', `Size', `Price', `Stock', `Price Update'], [`T-shirt', `Nike', `M', `25.00', `100', `20.00\%'], [`Jeans', ``Levi's'', `32', `59.00', `150', `-10.00\%'], [`Shoes', `Adidas', `8', `99.00', `80', `-45.00\%'], [`Bags', `Louis Vuitton', `Universal', `699.00', `20', `30.00\%'], [`Watches', `Omega', `Universal', `999.00', `10', `56.00\%']]\\
Action: delete\_batch with Action Input: \{``dimension'': ``row'', ``index\_list'': [3, 4, 5]\}\\
Observation: [[`Category', `Brand', `Size', `Price', `Stock', `Price Update'], [`T-shirt', `Nike', `M', `25.00', `100', `20.00\%'], [`Jeans', ``Levi's'', `32', `59.00', `150', `-10.00\%']]\\
Action: get\_value\_by\_formula with Action Input: \{``position\_list'': [``D2'', ``F2''], operator=``PRODUCT''\}\\
Observation: 5\\
Action: get\_value\_by\_formula with Action Input: \{``position\_list'': [``D3'', ``F3''], operator=``PRODUCT''\}\\
Observation: -5.9\\
Action: update\_range with Action Input: \{``start\_position'': ``D2'', ``end\_position'': ``D3'', values\_list=[[25.00 + 5], [59.00 - 5.9]]\}\\
Observation: [[`Category', `Brand', `Size', `Price', `Stock', `Price Update'], [`T-shirt', `Nike', `M', `30.00', `100', `20.00\%'], [`Jeans', ``Levi's'', `32', `53.10', `150', `-10.00\%']]\\
Action: finish with Action Input: \{\}\\
Observation: [[`Category', `Brand', `Size', `Price', `Stock', `Price Update'], [`T-shirt', `Nike', `M', `30.00', `100', `20.00\%'], [`Jeans', ``Levi's'', `32', `53.10', `150', `-10.00\%']]\\

\end{tcolorbox}
\begin{figure}[!h]
    \vspace{-0.08cm}
    \caption{Prompt details for Sheet.}
    \label{fig:sheet_prompt}
\end{figure}

==> prompt/weather.tex <==
\begin{tcolorbox}[breakable,title=Prompt Details for Weather]
\textbf{\textcolor{blue}{System Prompt}}\\ 
You can use actions to help people solve problems.\\
\begin{tikzpicture}
\draw[dashed] (0,0) -- (\linewidth,0); % 绘制一条宽度为\linewidth的虚线
\end{tikzpicture}
\textbf{\textcolor{blue}{Instruction}}\\
We detail name, description, input(parameters) and output(returns) of each action as follows:\\
Name: get\_user\_current\_date()\\
Description: Get the user's current date.\\
Returns:\\
The current date in `YYYY-MM-DD' format.\\
\\
Name: get\_user\_current\_location()\\
Description: Get the user's current city.\\
Returns:\\
The user's current city.\\
\\
Name: get\_historical\_temp(latitude, longitude, start\_date, end\_date)\\
Description: Get historical temperature data for a specified location and date range.\\
Parameters:\\
- latitude (Type: number): The latitude of the location.\\
- longitude (Type: number): The longitude of the location.\\
- start\_date (Type: string): The start date of the historical data (YYYY-MM-DD).\\
- end\_date (Type: string): The end date of the historical data (YYYY-MM-DD).\\
Returns:\\
Historical temperature data.\\
\\
Name: get\_historical\_rain(latitude, longitude, start\_date, end\_date)\\
Description: Get historical rainfall data for a specified location and date range.\\
Parameters:\\
- latitude (Type: number): The latitude of the location.\\
- longitude (Type: number): The longitude of the location.\\
- start\_date (Type: string): The start date of the historical data (YYYY-MM-DD).\\
- end\_date (Type: string): The end date of the historical data (YYYY-MM-DD).\\
Returns:\\
Historical rainfall data.\\
\\
Name: get\_historical\_snow(latitude, longitude, start\_date, end\_date)\\
Description: Get historical snowfall data for a specified location and date range.\\
Parameters:\\
- latitude (Type: number): The latitude of the location.\\
- longitude (Type: number): The longitude of the location.\\
- start\_date (Type: string): The start date of the historical data (YYYY-MM-DD).\\
- end\_date (Type: string): The end date of the historical data (YYYY-MM-DD).\\
Returns:\\
Historical snowfall data.\\
\\
Name: get\_snow\_forecast(latitude, longitude, start\_date, end\_date)\\
Description: Get snowfall forecast data for a specified location and date range.\\
Parameters:\\
- latitude (Type: number): The latitude of the location.\\
- longitude (Type: number): The longitude of the location.\\
- start\_date (Type: string): The start date of the forecast (YYYY-MM-DD).\\
- end\_date (Type: string): The end date of the forecast (YYYY-MM-DD).\\
Returns:\\
Snowfall forecast data.\\
\\
Name: get\_current\_snow(latitude, longitude, current\_date)\\
Description: Get current snowfall data for a specified location and date.\\
Parameters:\\
- latitude (Type: number): The latitude of the location.\\
- longitude (Type: number): The longitude of the location.\\
- current\_date (Type: string): The current date to retrieve snowfall data (YYYY-MM-DD).\\
Returns:\\
Current snowfall data.\\
\\
Name: get\_current\_temp(latitude, longitude, current\_date)\\
Description: Get current temperature data for a specified location and date.\\
Parameters:\\
- latitude (Type: number): The latitude of the location.\\
- longitude (Type: number): The longitude of the location.\\
- current\_date (Type: string): The current date to retrieve temperature data (YYYY-MM-DD).\\
Returns:\\
Current temperature data.\\
\\
Name: get\_latitude\_longitude(name)\\
Description: Get latitude and longitude information for a specified location name.\\
Parameters:\\
- name (Type: string): The name of the location. (e.g., city name)\\
Returns:\\
latitude and longitude information for the specified location.\\
\\
Name: get\_elevation(latitude, longitude)\\
Description: Get elevation data for a specified location.\\
Parameters:\\
- latitude (Type: number): The latitude of the location.\\
- longitude (Type: number): The longitude of the location.\\
Returns:\\
Elevation data for the specified location.\\
\\
Name: get\_temp\_forecast(latitude, longitude, start\_date, end\_date)\\
Description: Get temperature forecast data for a specified location and date range.\\
Parameters:\\
- latitude (Type: number): The latitude of the location.\\
- longitude (Type: number): The longitude of the location.\\
- start\_date (Type: string): The start date of the forecast (YYYY-MM-DD).\\
- end\_date (Type: string): The end date of the forecast (YYYY-MM-DD).\\
Returns:\\
Temperature forecast data.\\
\\
Name: get\_rain\_forecast(latitude, longitude, start\_date, end\_date)\\
Description: Get rainfall forecast data for a specified location and date range.\\
Parameters:\\
- latitude (Type: number): The latitude of the location.\\
- longitude (Type: number): The longitude of the location.\\
- start\_date (Type: string): The start date of the forecast (YYYY-MM-DD).\\
- end\_date (Type: string): The end date of the forecast (YYYY-MM-DD).\\
Returns:\\
Rainfall forecast data.\\
\\
Name: get\_current\_rain(latitude, longitude, current\_date)\\
Description: Get current rainfall data for a specified location and date.\\
Parameters:\\
- latitude (Type: number): The latitude of the location.\\
- longitude (Type: number): The longitude of the location.\\
- current\_date (Type: string): The current date to retrieve rainfall data (YYYY-MM-DD).\\
Returns:\\
Current rainfall data.\\
\\
Name: get\_distance(latitude1, longitude1, latitude2, longitude2)\\
Description: Calculate the distance between two sets of latitude and longitude coordinates.\\
Parameters:\\
- latitude1 (Type: number): The latitude of the first location.\\
- longitude1 (Type: number): The longitude of the first location.\\
- latitude2 (Type: number): The latitude of the second location.\\
- longitude2 (Type: number): The longitude of the second location.\\
Returns:\\
The distance between the two sets of coordinates in kilometers.\\
\\
Name: get\_historical\_air\_quality\_index(latitude, longitude, start\_date, end\_date)\\
Description: Get historical air quality index data for a specified location and date range.\\
Parameters:\\
- latitude (Type: number): The latitude of the location.\\
- longitude (Type: number): The longitude of the location.\\
- start\_date (Type: string): The start date of the historical data (YYYY-MM-DD).\\
- end\_date (Type: string): The end date of the historical data (YYYY-MM-DD).\\
Returns:\\
Historical air quality index (PM2.5) data.\\
\\
Name: get\_current\_air\_quality\_index(latitude, longitude, current\_date)\\
Description: Get current air quality index data for a specified location and date.\\
Parameters:\\
- latitude (Type: number): The latitude of the location.\\
- longitude (Type: number): The longitude of the location.\\
- current\_date (Type: string): The current date to retrieve air quality index data (YYYY-MM-DD).\\
Returns:\\
Current air quality index (PM2.5) data.\\
\\
Name: get\_air\_quality\_level(air\_quality\_index)\\
Description: Determine the air quality level based on the air quality index (AQI).\\
Parameters:\\
- air\_quality\_index (Type: number): The air quality index (AQI) value.\\
Returns:\\
The air quality level, which can be `good', `fair', `moderate', `poor', `very poor', or `extremely poor'.\\
\\
Name: check\_valid\_actions()\\
Description: Get supported actions for current tool.\\
Returns:\\
- actions (Type: array): Supported actions for current tool.\\
\\
Name: finish(answer)\\
Description: Return an answer and finish the task\\
Parameters:\\
- answer (Type: [`string', `number', `array']): The answer to be returned\\
\\
\\
If you want to get the latitude and longitude information of a city, you must call ``get\_latitude\_longitude'', do not generate it by yourself which maybe wrong.\\
If you are finished, you will call ``finish'' action\\
Please refer to the format of examples below to solve the requested goal. Your response must be in the format of ``Action: [your action] with Action Input: [your action input]''\\
\begin{tikzpicture}
\draw[dashed] (0,0) -- (\linewidth,0); % 绘制一条宽度为\linewidth的虚线
\end{tikzpicture}
\textbf{\textcolor{blue}{Examples}}\\
Goal: What is the lowest temperature yesterday?\\
\\
Action: get\_user\_current\_location with Action Input: \{\}\\
Observation: Shanghai\\
Action: get\_latitude\_longitude with Action Input: \{``name'': ``Shanghai''\}\\
Observation: \{`results': [\{`name': `Shanghai', `latitude': 31.22222, `longitude': 121.45806, `country\_code': `CN'\}, \{`name': `Shanghai', `latitude': 34.85009, `longitude': -87.08501, `country\_code': `US'\}, \{`name': `Cornelia', `latitude': 38.64363, `longitude': -93.73938, `country\_code': `US'\}]\}\\
Action: get\_user\_current\_date with Action Input: \{\}\\
Observation: 2015-01-02\\
Action: get\_historical\_temp with Action Input: \{``latitude'': 31.22222, ``longitude'': 121.45806, ``start\_date'': ``2015-01-01'', ``end\_date'': ``2015-01-01''\}\\
Observation: \{`latitude': 31.200005, `longitude': 121.5, `daily\_units': \{`time': `iso8601', `temperature\_2m\_max': `°C', `temperature\_2m\_min': `°C', `temperature\_2m\_mean': `°C'\}, `daily': \{`time': [`2015-01-01'], `temperature\_2m\_max': [4.3], `temperature\_2m\_min': [-3.6], `temperature\_2m\_mean': [-0.1]\}\}\\
Action: finish with Action Input: \{``answer'': -0.1\}\\
Observation: -0.1\\
\end{tcolorbox}
\begin{figure}[!h]
    \vspace{-0.08cm}
    \caption{Prompt Details for Weather.}
    \label{fig:weather_prompt}
\end{figure}

==> tables/main_results.tex <==
\begin{table}[t!]
\centering
\resizebox{0.8\textwidth}{!}{\begin{tabular}{@{}cl*{5}{d{4.4}}@{}}
\toprule
& \textbf{Model} & \multicolumn{1}{c}{\textbf{Embodied AI}} & \multicolumn{1}{c}{\textbf{Game}} & \multicolumn{1}{c}{\textbf{Web}} & \multicolumn{1}{c}{\textbf{Tool}} & \multicolumn{1}{c}{\textbf{Avg.} } \\ \midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Closed-sourced LLMs \end{tabular}} &  GPT-4  & 71.7/50.6 & 66.8/48.4 & 58.1/27.1 & 83.0/64.2 & 70.1/47.9 \\

 & Claude2 & 34.5/27.9 & 40.9/20.0 & 55.5/23.2 & 67.5/39.2 & 47.9/27.6\\
 
 & GPT-3.5-Turbo & 39.7/22.8 & 22.5/ \phantom{1} 5.0 & 51.0/19.8 & 53.4/26.3 & 41.4/18.9 \\
 
 & GPT-3.5-Turbo-16k  & 24.2/12.8 & 19.4/ \phantom{1} 1.7 & 48.7/17.0 & 49.2/23.4 & 34.1/13.6 \\
 
 & Text-Davinci-003 & 21.7/10.4 & 30.2/10.9 & 44.2/16.0 & 60.6/30.4 & 37.2/16.2 \\ \midrule
 
\multirow{7}{*}{Open-sourced LLMs}  
&Mistral-7b & 15.2/ \phantom{1} 5.5 & 7.8/ \phantom{1} 0.0 & 40.7/ \phantom{1} 7.6 & 29.9/ \phantom{1} 0.0 & 22.5/ \phantom{1} 3.5
\\

&Llama2-13b & 12.9/ \phantom{1} 4.5 & 5.3/ \phantom{1} 0.0 & 35.6/ \phantom{1} 6.4 & 33.1/ \phantom{1} 0.0 & 19.7/ \phantom{1} 3.4 \\

 & Llama2-70b  & 15.3/ \phantom{1} 7.5 & 8.0/ \phantom{1} 0.8 & 35.6/\phantom{1} 8.4 & 43.2/\phantom{1} 0.0 & 23.7/ \phantom{1} 4.5 \\
 
 & CodeLlama-13b  & 13.3/ \phantom{1} 8.9 & 4.7/ \phantom{1} 0.9 & 41.6/14.8 & 44.2/18.8 & 24.5/ 10.6 \\
 
 & CodeLlama-34b  & 11.6/ \phantom{1} 5.5 & 17.0/\phantom{1} 1.7 & 46.5/13.8 & 55.2/\phantom{1} 7.9 & 30.2/ \phantom{1} 7.0 \\
 
 & Vicuna-13b-16k   & 13.1/ \phantom{1} 3.0 & 11.3/ \phantom{1} 0.9 &  42.3/12.4 & 30.6/\phantom{1} 1.7 & 23.1/ \phantom{1} 4.3 \\
 
 & Lemur-70b  & 21.4/ \phantom{1} 5.4 & 9.9/ \phantom{1} 1.7 & 42.1/ \phantom{1} 7.4 & 58.6/21.7 &  31.7/ \phantom{1} 8.6 \\ 

  & DeepSeek-67b  & 34.1/17.7 & 17.8/ \phantom{1} 3.3 & 48.3/18.8 & 55.9/28.8 &  38.5/17.2 \\ 
 
 \bottomrule
 \end{tabular}}
 
\caption{Performance of different LLMs across various categories. The ``Avg." represents the average calculated over all tasks in 9 environments. ``A/B" indicates that both ``progress rate" and ``success rate" are reported.}
\label{tab: results of different categories}
\end{table}

==> tables/subgoal_annotation.tex <==

\begin{table}[t!]
\centering
\footnotesize
\begin{tabular}{p{2.0cm}p{5.25cm}p{5.25cm}}
\toprule
\textbf{Task} & \textbf{Goal} & \textbf{Subgoals} \\ \midrule
AlfWorld
&
look at bowl under the desklamp.
&
Subgoal 1: \textasciicircum(?=.* you see)(?=.*a bowl \textbackslash d+) \newline
Subgoal 2: You pick up the bowl \textbackslash d+ \newline
Subgoal 3: \textasciicircum(?=.* you see)(?=.*a desklamp)
\\
\midrule
ScienceWorld
&
Your task is to find the animal with the longest life span. The animals are in the `outside' location. Focus on the animal with the longest life span.
&
Subgoal 1: You move to the outside.\newline
Subgoal 2: You focus on the crocodile egg.
\\
\midrule

BabyAI
&
go to the red ball
&
Subgoal 1: There is a red ball ** \newline
Subgoal 2: There is a red ball ** right in front of you 1 steps away.
\\
\midrule
Jericho
&
Get out of the house. Then escape the city without getting caught via driving.
&
Subgoal 1: You get out of bed. \newline
Subgoal 2: Bathroom This is a far from luxurious but still quite functional bathroom, with a sink, toilet and shower. The bedroom lies to the north. \newline
Subgoal 3: You step into the shower, turn on the water, and within a few moments you feel like a new man. But no time to dawdle - you hop back out again and dry off in record time. \newline
Subgoal 4: You put on the clean clothing. \newline
Subgoal 5: You open the front door. \newline
Subgoal 6: You climb inside and start up the engine. \newline
Subgoal 7: You have left Las Mesas
\\
\midrule
PDDL
&
The goal is to satisfy the following conditions: ball1 is at roomb. ball2 is at roomb. ball3 is at roomb. ball4 is at roomb.
&
	
Subgoal 1: ball1 is at roomb. \newline
Subgoal 2: ball2 is at roomb. \newline
Subgoal 3: ball3 is at roomb. \newline
Subgoal 4: ball4 is at roomb.
\\
\bottomrule
\end{tabular}
\caption{Examples of goals and subgoals for Embodied AI tasks~(AlfWorld, ScienceWorld and BabyAI).}
\label{tab:subgoal_annotation_1}
\end{table}


\begin{table}[t!]
\centering
\footnotesize
\begin{tabular}{p{2.0cm}p{5.25cm}p{5.25cm}}
\toprule
\textbf{Task} & \textbf{Goal} & \textbf{Subgoals} \\ \midrule
Tool-Query (Academia)
&
How many mutual collaborators do Florian Kirchbuchner and Fadi Boutros share? Please give me a numerical value as an answer.
&
Subgoal 1: AuthorNet is loaded. \newline
Subgoal 2: [`Fadi Boutros', `Naser Damer', `Arjan Kuijper', 'Meiling Fang'] \newline
Subgoal 3: ['Naser Damer', 'Florian Kirchbuchner', 'Arjan Kuijper'] \newline
Subgoal 4: 2
\\
\midrule
Tool-Query (Movie)
&
Is the movie `Disenchanted' a Japanese film? Answer Yes or No.
&
Subgoal 1: [\{`id': 338958, `title': `Disenchanted'\}] \newline
Subgoal 2: \{`production\_countries': [\{`iso\_3166\_1': `US', `name': `United States of America'\}]\} \newline
Subgoal 3: No
\\
\midrule
Tool-Query (Weather)
&
Which day had a greater amount of rainfall, the 7th of last month or the 20th of last month? Please provide the answer in the YYYY-MM-DD format.
&
Subgoal 1: 2015-05-15 \newline
Subgoal 2: Pittsburgh \newline
Subgoal 3: \{`results': [\{`name': `Pittsburgh', `latitude': 40.44062, `longitude': -79.99589, `country\_code': `US'\}, \{`name': `Hymera', `latitude': 39.18643, `longitude': -87.30168, `country\_code': `US'\}, \{`name': `Tipton', `latitude': 39.34307, `longitude': -98.4709, `country\_code': 'US'\}]\} \newline
Subgoal 4: \{`latitude': 40.40001, `longitude': -80.0, `daily\_units': \{`time': `iso8601', `rain\_sum': `mm'\}, `daily': \{`time': [`2015-04-07'], `rain\_sum': [9.6]\}\} \newline
Subgoal 5: \{`latitude': 40.40001, `longitude': -80.0, `daily\_units': \{`time': `iso8601', `rain\_sum': `mm'\}, `daily': \{`time': [`2015-04-20'], `rain\_sum': [17.6]\}\} \newline
Subgoal 6: 2015-04-20
\\
\midrule
Tool-Operation (Todo)
&
Finally, I have completed the task Read and summarize a history chapter, please mark it as completed.
&
Subgoal 1: [\{`order': 1, `color': `charcoal', `name': `Homework and Assignments', `is\_favorite': False\}, \{`order': 2, `color': `charcoal', `name': `Extracurricular Activities', `is\_favorite': False\}] \newline
Subgoal 2: [\{`order': 1, `content': `Solve algebra equations', `is\_completed': False, `priority': 1, `due\_date': `2015-06-01'\}, \{`order': 2, `content': `Conduct a chemistry experiment', `is\_completed': False, `priority': 2, `due\_date': `2015-06-12'\}, \{`order': 3, `content': `Read and summarize a history chapter', `is\_completed': False, `priority': 3, `due\_date': `2015-06-06'\}] \newline
Subgoal 3: \{`message': `Complete task successfully.', `task': \{`order': 3, `content': `Read and summarize a history chapter', `priority': 3, `due\_date': `2015-06-06'\}\}
\\ 
\bottomrule
\end{tabular}
\caption{Examples of goals and subgoals for Tool-Query tasks~(Academia, Movie and Weather) and Tool-Operation tasks~(Todo).}
\label{tab:subgoal_annotation_3}
\end{table}



\begin{table}[t!]
\centering
\footnotesize
\begin{tabular}{p{2.0cm}p{5.25cm}p{5.25cm}}
\toprule
\textbf{Task} & \textbf{Goal} & \textbf{Subgoals} \\ \midrule
Jericho
&
Get out of the house. Then escape the city without getting caught via driving.
&
Subgoal 1: You get out of bed. \newline
Subgoal 2: Bathroom This is a far from luxurious but still quite functional bathroom, with a sink, toilet and shower. The bedroom lies to the north. \newline
Subgoal 3: You step into the shower, turn on the water, and within a few moments you feel like a new man. But no time to dawdle - you hop back out again and dry off in record time. \newline
Subgoal 4: You put on the clean clothing. \newline
Subgoal 5: You open the front door. \newline
Subgoal 6: You climb inside and start up the engine. \newline
Subgoal 7: You have left Las Mesas
\\
\midrule
PDDL
&
The goal is to satisfy the following conditions: ball1 is at roomb. ball2 is at roomb. ball3 is at roomb. ball4 is at roomb.
&
	
Subgoal 1: ball1 is at roomb. \newline
Subgoal 2: ball2 is at roomb. \newline
Subgoal 3: ball3 is at roomb. \newline
Subgoal 4: ball4 is at roomb.
\\
\bottomrule
\end{tabular}
\caption{Examples of goals and subgoals for Game tasks~(Jericho and PDDL).}
\label{tab:subgoal_annotation_2}
\end{table}


% \begin{table}[t!]
% \centering
% \footnotesize
% \begin{tabular}{p{1.5cm}p{2.25cm}p{9.0cm}}
% \toprule
% \textbf{Task}  & \textbf{Goal} & \multicolumn{1}{c}{\textbf{Trajectory}}\\
% \midrule
% \multirow{1}[0]{*}{AlfWorld} 
% % AlfWorld
% &
% \multirow{1}[0]{2.25cm}{put two soapbar in garbagecan.}
% % put two soapbar in garbagecan.
% &
% Step: \textcolor{red}{0} \ \
% Action: \textcolor{violet}{open cabinet 4}\ \
% Observation: \textcolor{orange}{You open the cabinet 4. The cabinet 4 is open. In it, you see a soapbar 2.}\ \
% PR: \textcolor{blue}{0.25}

% ...

% Step: \textcolor{red}{19}\ \
% Action: \textcolor{violet}{put soapbar 1 in/on garbagecan 1}\ \
% Observation: \textcolor{orange}{You put the soapbar 1 in/on the garbagecan 1.}\ \
% PR: \textcolor{blue}{1.0}
% \\
% \midrule
% \multirow{1}[0]{*}{ScienceWorld} 
% % AlfWorld
% &
% Your task is to find the animal with the longest life span.  The animals are in the 'outside' location.  Focus on the animal with the longest life span.
% % put two soapbar in garbagecan.
% &
% ...

% Step: \textcolor{red}{5}
% Action: \textcolor{violet}{go to outside}
% Observation: \textcolor{orange}{You move to the outside.}
% PR: \textcolor{blue}{0.5}

% ...

% Step: \textcolor{red}{7}
% Action: \textcolor{violet}{focus on crocodile egg}
% Observation: \textcolor{orange}{You focus on the crocodile egg.}
% PR: \textcolor{blue}{1.0}
% \\
% \midrule
% \multirow{1}[0]{*}{BabyAI} 
% &
% go to the red ball
% &
% ...

% Step: \textcolor{red}{13}
% Action: \textcolor{violet}{turn right}
% Observation: \textcolor{orange}{In front of you in this room, you can see several objects: There is a grey ball 1 2 steps in front of you and 1 steps to your right. ... You are carrying a grey key.}
% PR: \textcolor{blue}{0.5}

% Step: \textcolor{red}{14}
% Action: \textcolor{violet}{go to red ball 1}
% Observation: \textcolor{orange}{In front of you in this room, you can see several objects: There is a red ball 1 right in front of you 1 steps away. There is a grey key 1 0 steps in front of you and 1 steps to your right. There is a grey box 1 0 steps in front of you and 2 steps to your right. ... You are carrying a grey key. The task is completed.}
% PR: \textcolor{blue}{1.0}
% \\
% \midrule
% \multirow{1}[0]{*}{Jericho} 
% &
% search for a mug in an inn. 
% &
% ...

% Step: \textcolor{red}{1}
% Action: \textcolor{violet}{East}
% Observation: \textcolor{orange}{Inside the Inn There are a few patches of mould on the walls and the floorboards creak slightly, but the building seems safe enough. As you move you disturb a thin layer of dust. There are some stone steps leading down, and an open doorway to the outside to the west. You see some tables and chairs. There is a dark, intricately-carved wooden chair in the corner behind you. You can go west (back outside) or down some steps. You can see a magnificently carved chair here.}
% PR: \textcolor{blue}{0.33}

% ...

% Step: \textcolor{red}{5}
% Action: \textcolor{violet}{Examine barrels}
% Observation: \textcolor{orange}{The barrels are now no more than rotten staves of dry wood, held together by the woodworm holding hands. You have found a pewter mug...}
% PR: \textcolor{blue}{1.0}
% \\
% \bottomrule
% \end{tabular}
% \caption{Examples of goals and subgoals for Embodied AI tasks~(AlfWorld, ScienceWorld and BabyAI).}
% \label{tab:subgoal_annotation_4}
% \end{table}




==> tables/tool_comparison.tex <==
% \begin{table*}[!t]
%     \centering
%     \small
%     \resizebox{0.95\linewidth}{!}{
%     \begin{tabular}{lccccc}
%         \toprule
%         \textbf{Resource} & \textbf{Ours}& \textbf{AgentBench} & \textbf{ToolEval}  & 
%         \textbf{API-Bank} &  \textbf{ToolAlpaca}   
%         \\
%         \midrule
%           Real-world API?   & \cmark &  &  &  &   \\ 
%           Real API Call\&Response? & \cmark &  &  &  &   \\ 
%           Multi-step Reasoning?  & \cmark &  &  &  &   \\
%           Operation? & \cmark & & & & \\
%           Fine-grained Evaluation? & & & &  & \\
%          \bottomrule
%     \end{tabular}
%     }
%     \caption{
%     \small{A comparison of our XXX to notable instruction tuning dataset for tool learning.
%     }
%     }
%     \label{tab:dataset_comparison}
% \end{table*}

==> tables/tool_environment.tex <==
% \begin{table}[t]
% \centering
% \setlength\tabcolsep{3pt}
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Datasets} & \textbf{Category} & \textbf{\# Actions} & \textbf{$\boldsymbol{\bar{N}_{\text{subgoals}}}$} & \textbf{$\boldsymbol{\bar{N}_{\text{categories}}}$} \\
% \midrule
% Weather  & Query       & 19   & 6.1      & 5.1      \\
% Movie    & Query       & 16   & 4.3      & 3.6        \\
% Academia & Query      & 9    & 5.6     & 4.0     \\
% Todo     & Operation  & 12   & 4.8     & 3.6      \\
% Sheet    & Operation  & 19   & 5.8     & -     \\
% \bottomrule
% \end{tabular}
% \caption{
% Tool-using test datasets investigated in this work.
% We report the average number of subgoals ($\bar{N}_{\text{subgoals}}$), average number of action categories ($\bar{N}_{\text{categories}}$).
% % report number of steps
% \label{tab:tool_environment} 
% }
% \end{table}
